Wavefront Sets of Unipotent Representations of Reductive $p$-adic Groups II

The wavefront set is a fundamental invariant of an admissible representation arising from the Harish-Chandra-Howe local character expansion. In this paper, we give a precise formula for the wavefront set of an irreducible representation of real infinitesimal character in Lusztig's category of unipotent representations in terms of the Deligne-Langlands-Lusztig correspondence. Our formula generalizes the main result of arXiv:2112.14354, where this formula was obtained in the Iwahori-spherical case. We deduce that for any irreducible unipotent representation with real infinitesimal character, the algebraic wavefront set is a singleton, verifying a conjecture of M\oeglin and Waldspurger. In the process, we establish new properties of the generalized Springer correspondence in relation to Lusztig's families of unipotent representations of finite reductive groups.

==> scratch.tex <==



    We have that $\lambda^t = (A_i^{\bar\lambda_i})_i$.
    Moreover $A_i \equiv \#\{j\mid f(j)\ge i\}\pmod 2$.
    Thus if we set $\mathcal S' = \bigcup_{i=0}^{l-1}(f(2i),f(2i+1)]$ then $A_i\equiv N\pmod 2$ if and only if $i\in \mathcal S'$.
    Now suppose first that $N$ is odd.
    Then $d(\lambda) = ((\lambda^t)_-)_C$ and the odd entries of $\lambda^t$ are $(A_i^{\bar\lambda_i})_{i\in \mathcal S'}$.
    We also have for $i\in \mathcal S'$, $\bar \lambda_i$ is even if and only if $i\in (1,f(1))\cup\bigcup_{i=1}^{l-1}(f(2i)+1,f(2i+1))\cup\{f(2i+1)\mid f(2i)+1 = f(2i+1)\}$.
    Thus if we pair off the odd entries of $(\lambda^t)_-$ the pairs with unequal entries are precisely $(A_{f(2i-1)},A_{f(2i)+1})$ for $1\le i<l$ and, when $f(2l-1)\ne k$, $(A_{f(2l-1)},A_{f(2l)}-1)$.
    Since $a_{f(i)} = 1$ for all $i$, we have that $A_{f(2i-1)}-1 = A_{f(2i-1)+1}$ and $A_{f(2i)+1}+1 = A_{f(2i)}$.
    Thus $d(\lambda) = (A_i^{\bar\lambda_i+\tilde \delta})$ where $\tilde\delta$ at indices $[f(2i-1),f(2i)+1]$ is $(-1,1,0,\dots,0,1,-1)$ when $f(2i-1)+1<f(2i)$, and ????
